The Fermi Large Area Telescope On Orbit: Event Classification, Instrument Response Functions, and Calibration

The Fermi Large Area Telescope (Fermi-LAT, hereafter LAT), the primary instrument on the Fermi Gamma-ray Space Telescope (Fermi) mission, is an imaging, wide field-of-view, high-energy \gamma-ray telescope, covering the energy range from 20 MeV to more than 300 GeV. During the first years of the mission the LAT team has gained considerable insight into the in-flight performance of the instrument. Accordingly, we have updated the analysis used to reduce LAT data for public release as well as the Instrument Response Functions (IRFs), the description of the instrument performance provided for data analysis. In this paper we describe the effects that motivated these updates. Furthermore, we discuss how we originally derived IRFs from Monte Carlo simulations and later corrected those IRFs for discrepancies observed between flight and simulated data. We also give details of the validations performed using flight data and quantify the residual uncertainties in the IRFs. Finally, we describe techniques the LAT team has developed to propagate those uncertainties into estimates of the systematic errors on common measurements such as fluxes and spectra of astrophysical sources.

==> aeff_diagnostic.tex <==
\subsection{Studies with diagnostic event streams}



==> aeff_triggerRateDep.tex <==
\subsection{Trigger rate dependence}



==> bkg_errorAnalysis.tex <==
%\subsection{Residual Particle Background Contamination in High-Purity Event Samples}\label{subsec:bkg_errors}






==> edisp_bracketStudy_eDisp_B21520p31.tex <==
Bracketing \aeff & $N_{0}$ & $\alpha$ & $\beta$ & $F_{25}$ & $S_{25}$ \\
 & [MeV$^{-1}$ cm$^{-2}$ s$^{-1}$] & & & [cm$^{-2}$ s$^{-1}$] & [MeV cm$^{-2}$ s$^{-1}$] \\
\hline
\hline
Nominal & $5.23 \times 10^{-10}$ & 2.24 & 0.08 & $4.09 \times 10^{-7}$ & $1.33 \times 10^{-4}$ \\
\bracketirf{E_{disp}} & $5.43 \times 10^{-10}$ & 2.20 & 0.10 & $4.14 \times 10^{-7}$ & $1.35 \times 10^{-4}$ \\


==> edisp_bracketStudy_eDisp_PG1553p133.tex <==
Bracketing \aeff & $N_{0}$ & $\Gamma$ & $F_{25}$ & $S_{25}$ \\
 & [MeV$^{-1}$ cm$^{-2}$ s$^{-1}$] & & [cm$^{-2}$ s$^{-1}$] & [MeV cm$^{-2}$ s$^{-1}$] \\
\hline
\hline
Nominal & $2.54 \times 10^{-12}$ & 1.68 & $6.91 \times 10^{-8}$ & $1.19 \times 10^{-4}$\\
\bracketirf{E_{disp}} & $2.60 \times 10^{-12}$ & 1.69 & $7.13 \times 10^{-8}$ & $1.21 \times 10^{-4}$\\


==> edisp_unfolding.tex <==
\subsection{Using Unfolding Techniques to Treat the LAT Energy Response in Spectral Fitting}%
\label{subsec:EDisp_unfolding}

Spectral unfolding (deconvolution) is an approach for taking the energy
dispersion into account in the spectral fitting. Unfolding is in effect the
opposite of the \emph{forward folding} approach implemented in many popular
astronomical data analysis packages (and used in the standard likelihood
point source analysis implemented in the \stools), where the 
IRFs are folded with the spectral model and the model parameters
are varied until the best match with the measured count spectrum is
found---e.g., this is how XSPEC~\citep{REF:xspec} handles the energy dispersion.

Energy unfolding has been used for several analyses of LAT data, mainly to
cross-check the results of the standard likelihood
analysis~\citep{REF:BlazarSEDs} and especially for the lowest or
highest energies: below $\sim 100$~MeV~\citep{CrabPaper} or above
$\sim 100$~GeV~\citep{REF:2010.CREPRD,REF:2009.Electrons20GeV1TeV}.
The Bayesian approach detailed in~\citet{REF:BayesUnfolding} is that typically
being used by the LAT Collaboration.
Compared to other popular algorithms---most notably the Singular Value
Decomposition (SVD) approach~\citep{REF:SVDUnfolding}---it has the advantage
that it does not require matrix inversions and can be easily generalized to
multidimensional problems (e.g., when unfolding in energy and angle is needed).
In addition to that rigorous prescriptions are available in this framework 
to take the systematic uncertainties into account in the spectral analysis.

The unfolding algorithms mentioned above are implemented and available
in the public domain in several different analysis
frameworks, \citep[e.g.,][]{REF:RooUnfold}.
The reader is referred to \citet{UnfoldingMazziotta} for a more comprehensive
introduction to the spectral unfolding techniques in the context of the LAT
data analysis.


==> perf_perf_spatialExtent.tex <==
\subsection{Source Extension}\label{subsec:perf_spatialExtent}

As was discussed in \secref{subsec:PSF_onextension},
studying the spatial extension of \gammaRayHyph\ sources in the LAT data is important for several reasons
and many spatially-extended sources have now been detected by the LAT.

The strong energy dependence of the PSF of the LAT makes the study of source extension a delicate issue. 
The larger PSF at low energies implies that soft sources will be harder to resolve. Furthermore, as was 
shown in \secref{subsec:PSF_onextension}, an incorrect model of the PSF
  can bias the significance of the detection of the extension of a source.
  Therefore, it is important to use the most accurate available representation of the PSF when studying spatially-extended
  sources.

%\item The likelihood-ratio test can only be used to compute the statistical
%  significance of the extension of a source when the two models are nested
%  and when all of the parameters of the two models are simultaneously maximized.
%  In particular, when comparing to the likelihood of a point-like source,
%  it is important to refit the point-like source's position to avoid
%  biasing the statistical significance.
%\item Any imperfection in the model of the Galactic diffuse emission can pose
%  a serious problem for nearby sources; for best results a dedicated
%  re-analysis of the diffuse emission in the region may boost the effectiveness
%  of an extension test.


The sensitivity to the spatial extension of a \gammaRayHyph\ source is defined as the
minimum flux required to resolve the extension of a source.  
In \citet{REF:SourceExt}, the
LAT sensitivity to spatial extension was computed using a dedicated
MC study for a variety of time ranges, spectral models,
background levels, and energy ranges. Here, we show the sensitivity
for one representative set of parameters.

\begin{figure}[htb!]
  \centering
  \includegraphics[width=\onecolfigwidth]{extension_sensitivity}
  \caption{
  (a) The minimum flux for which an extended source can be spatially resolved as
  a function of the extension of the source for a ten year exposure.
  The sensitivity is computed and the flux is integrated in the 1~GeV to
  100~GeV energy range.  
  The sensitivity is
  computed for sources with power-law spectral model of
  spectral index 2 against a background
  representative of the Galactic plane.  The gray region brackets the
  projected sensitivity assuming that the sensitivity increases from
  2 to 10 years by the square root of the exposure and
  linearly in the exposure.  (b) The factor increase in sensitivity
  for a 10 year exposure compared to a 2 year exposure. This plot is
  adapted from \citet{REF:SourceExt}.
  }
  \label{fig:perf_spatialExtent}
\end{figure}

\figref{perf_spatialExtent} compares the 2 year and 10 year sensitivity
of the LAT to the spatial extension of a source.  The plot shows that
the sensitivity of the LAT to the extension of a source is poor when
the size of the source is comparable to the size of the high-energy
PSF of the LAT.  On the other hand, the sensitivity of the LAT
to these smaller sources increases over time by a factor greater than
the square root of the exposure time.  This is because the extension is
measured most sensitively with by high-energy \gammaRays\ and the 
intensity of the diffuse background decreases rapidly with energy.
For larger sources, the sensitivity increase is more modest because
the effective background counts increases with the size of the source.  






